ARGUS: Visualization of AI-Assisted Task Guidance in AR

The concept of augmented reality (AR) assistants has captured the human imagination for decades, becoming a staple of modern science fiction. To pursue this goal, it is necessary to develop artificial intelligence (AI)-based methods that simultaneously perceive the 3D environment, reason about physical tasks, and model the performer, all in real-time. Within this framework, a wide variety of sensors are needed to generate data across different modalities, such as audio, video, depth, speech, and time-of-flight. The required sensors are typically part of the AR headset, providing performer sensing and interaction through visual, audio, and haptic feedback. AI assistants not only record the performer as they perform activities, but also require machine learning (ML) models to understand and assist the performer as they interact with the physical world. Therefore, developing such assistants is a challenging task. We propose ARGUS, a visual analytics system to support the development of intelligent AR assistants. Our system was designed as part of a multi year-long collaboration between visualization researchers and ML and AR experts. This co-design process has led to advances in the visualization of ML in AR. Our system allows for online visualization of object, action, and step detection as well as offline analysis of previously recorded AR sessions. It visualizes not only the multimodal sensor data streams but also the output of the ML models. This allows developers to gain insights into the performer activities as well as the ML models, helping them troubleshoot, improve, and fine tune the components of the AR assistant.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January 2022

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> text/old-03-overview.tex <==
\section{Background: Building The TIM Personal Assistant}
\label{sec:overview}

In this section, we describe the context of the development of \systemname. This includes the ecosystem of components needed to support intelligent AR assistant systems, spanning from software running on headset device to data management modules able to ingest data in real-time.

\subsection{Motivating Context}
The development of \systemname is driven in large part by the requirements of DARPA's Perceptually-enabled Task Guidance (PTG) program \cite{darpaptgbaa}. PTG aims to develop AI technologies to help users perform complex physical tasks while making them more versatile by expanding their skillset and more proficient by reducing their errors \cite{ptg_site}. PTG seeks to develop methods, techniques, and technology for artificially intelligent assistants that provide just-in-time visual and audio feedback to help with task execution. The goal is to provide users of PTG assistants with wearable sensors (head-mounted cameras and microphones) that allow the assistant to see what they see and hear and what they hear, and augmented reality (AR) headsets that allow assistants to provide feedback through speech and aligned graphics. The assistants learn about tasks by ingesting knowledge from checklists, illustrated manuals, training videos, and other sources of information (e.g., making a meal from a recipe, applying a tourniquet from directions, conducting a pre-flight check from checklist). They then combine this task knowledge with a perceptual model of the environment to support mixed-initiative and task-focused user dialogs. The dialogs may assist a user in completing a task, identifying and correcting an error during a task and instructing them through a new task taking into consideration the user’s level of expertise.

\subsection{Transparent, Interpretable, and Multimodal Personal Assistant}







\textit{ARGUS} works with an assistive AR framework (TIM) that integrates perceptual grounding, attention and user modeling during real-time AR tasks. 

\textbf{Architecture}
TIM works with \systemname via a WebSocket network and it streams its on-board sensor data (i.e., gaze, hand tracking, see details in the subsection below) in real-time. This allows us to shift the computation heavy tasks to the server while keep the essential tasks on the Hololens to improve responsiveness. The sensory data are fist compressed to save the network usage and decompress later for further analysis. It also collects the machine learning prediction results from the server and updates the AR interaction and interface accordingly. The AR client running on the Hololens takes two streaming to support contextual interaction: a \textit{reasoning} stream that recognizes users actions and a \textit{perception} stream that recognizes objects in the scene. On average, these streams takes about 100ms to complete one update cycle to the AR client.

\comment{
\textbf{Role of \systemname}
In a high-level, \textit{\systemname} helps users to see and hear the otherwise invisible data and calculations happening in an assistive AR system. 
By visualizing the video feed, 3D reconstructions and sensory data, The dashboard visualizations in \textit{ARGUS} makes TIM \textit{transparent} and \textit{interpretable} since showing the raw information in realtime is designed to help the user understanding what happens on the assistive AR system in realtime interaction. Unlike most machine learning models that output the predictions from raw data (less transparent), \textit{ARGUS} visualizes these raw data alone with machine learning predictions for better transparency. Finally, TIM is \textit{multimodal} as it takes in various inputs such as gestures,gaze and voice and outputs both visual and auditory feedback to users. 

\michael{I think this again focuses on \systemname too much. At this point, we just want to describe the AR assitant (TIM) and the infrastructure. }
}


\subsection{Modeling}
\label{subsec:modeling}
\myparagraph{Perception}

\chen{Iran and Bea, could you also mention the hand detection model here?} 

This module uses multimodal machine-sensing models to detect human-object interactions in the environment. The output is real-time estimations with model confidence levels of three environmental elements: object categories, object localizations, and human action detections. We modulate object outputs via text instructions, allowing us to selectively detect objects and actions that are part of a particular procedure (i.e. recipe) and disregard everything else. To achieve this, our models generate and compare text and sensor (i.e. RGB camera) representations. Next we describe the main features of the models that we use.

\textit{Object detection and localization}. We use Detic \cite{zhou2022detecting} to generate these estimations, as it is a model that encodes in parallel RGB frames and free-form text descriptions of objects of interest (i.e. ``the blue cup'') and it generates bounding-box and object mask estimations for the regions in the frame where the objects are detected. Its direct comparison of RGB and text modalities is enabled via contrastive language-image pre-training (CLIP) \cite{radford2021learning}.

\textit{Action recognition}. We allow ARGUS users to select between three action-recognition models: Omnivore \cite{girdhar2022omnivore}, SlowFast \cite{xiao2020audiovisual,kazakos2021slow,feichtenhofer2019slowfast} and EgoVLP \cite{qinghong2022egocentric}. 
\michael{Again do not mention \systemname yet -- and I think that this should be TIM anyway, right? The AR assistant (TIM) can choose between the different recognition models.}
These process video streams to output verb-noun tuples that describe actions, each with its own benefits and limiations. 
While Omnivore is considered state-of-the-art for action recognition, it is a classification model with a fixed vocabulary. EgoVLP is has a joint RGB-text representation that, similar to Detic and CLIP, allows for the detection of free-form text descriptions of actions. SlowFast integrates audio and RGB information, allowing to potentially detect actions outside the RGB field of view. Therefore, each model may be optimal in different deployment conditions. 

We also trained a gated recurrent unit (GRU) \cite{cho2014learning} that takes all perception models' instantaneous encodings to integrate them over time and generate real-time estimations of the current procedural step being carried out by the human performer.

\myparagraph{Reasoning and Knowledge Transfer}
\claudio{maybe use ``task description'' versus ``recipe''}
%\chen{add here}
Reasoning and knowledge transfer first preprocesses the input task description, and output the necessary objects and actions for each step. Then for each frame, it
takes the object and action outputs from the perceptual grounding component along with the processed input task description, and makes two decisions:
\textbf{Error detection} detects whether the user makes an error in the current frame; \textbf{Step prediction} predicts whether the current step is complete and should move to the next step.

\textit{Error detection}. We check whether these certain objects and actions processed from the task description are detected in the scene using the outputs from Perception. If not, we decide that the user makes an error in this frame. 

\chen{For step prediction, I keep it simple and do not add other low-level implementations in this paragraph.}
\textit{Step prediction}. We use an off-the-shelf hands detection model, and the system decides to move into the next step if hands are not detected for more than five seconds.


\subsection{System Architecture}
\label{subsec: dashboard_arquitecture}
% \bea{add here. please feel free to reorganize this section}

To enable data streaming capabilities, the system utilizes server-side infrastructure that provides a centralized data communication hub and real-time machine learning inference to facilitate ingesting, operating over, and contextualizing the produced data streams. A system diagram can be seen in Figure~\ref{fig:architecture}.
% a message-hub for inter-component communication, as well as different computational modules \bea{bea fix wording} that provide machine learning and contextualize the data in the 3D environment.

% The high-level architecture of \systemname \michael{This seems to be confusing to me. \systemname is the debugging tool explained in \autoref{sec:system}, but we explain the AR assistant here, so should this say "The high-level architecture of TIM (Transparent, Interpretable, and Multimodal Personal Assistant)"? I guess it makes sense to explain the infrastructure here, but I would not mention \systemname already.} is depicted in Figure~\ref{fig:architecture}. 
% In what follows, we describe its key components.
%
\begin{figure}
    \centering
    \includegraphics[width=0.44\textwidth]{figs/imgs/simple_arch.png}
    \vspace{-.2cm}
    \caption{The System's backend architecture that acts as a data communication service between the system components: the Hololens, the AI and computational components, and the \systemname dashboard.
    \label{fig:architecture}}
    \vspace{-.5cm}
\end{figure}
%

% \myparagraph{Human Interfaces}
% \systemname is one of the human interfaces that allow the user to explore the data. Besides \systemname, HoloLens user and other developer tools are supported.
% \michael{See above -- I think we should mention \systemname here yet, but just explain the rest of the architecture that is then later accessed/used by \systemname. This section here should just explain TIM and the rest of the infrastructure.}

\myparagraph{Data Orchestration and Storage}
The core of our architecture is Redis Streams, which we use as our data message queue. We have a REST+Websocket API to provide a uniform abstraction layer for components to interact with. 
% that we wrap around Redis so that our other components can be independent to server-side internals.
The HoloLens streams its sensor data to the API where it is made available to all of the other components in our system. 
The user is able to record data streaming sessions, which will listen and copy all data streams to disk.
% If the user is recording, the recorders will listen and produce a copy of the data to disk.
Then in the future, we can selectively replay that data back into the system as if the HoloLens was running for easier offline testing.

\myparagraph{AI resources}
The task guidance system has multiple AI components that perform understanding of the incoming data streams. 
% The perception component is responsible for characterizing and communicating the current state of the task and its entities.
% The memory component takes perception outputs and integrates them into a model of the 3D environment.
% Taking a look at the AI side, the dotted arrows on the right (see Figure~\ref{fig:architecture}) are to show how the traffic is actually flowing, but the solid arrows can just be followed to understand the data pipeline. 
As AI resources, we have three modules: (1) Perception utilizes information from historical instances of these actions and actions from similar tasks and makes its best prediction of what the current action and objects are. (2) Memory takes the objects and transforms them into 3D coordinates and contextualizes objects over time in the 3D environment. (3) Reasoning then uses those objects and the actions returned by perception to understand whether the user is performing the recipe correctly. Any of this data can be picked up and shown on our dashboard, or even in the Hololens AR user interface and command line tools.


\subsection{Data}
\label{subsec: data}

HoloLens 2 can provide various data from multiple sensors on board. 
With HoloLens 2 research mode enable, we stream the data from the main RGB camera, 4 grayscale cameras, infrared depth camera and IMU which contains accelerometer, gyroscope and magnetometer. 
The data format of the image sensors can be found at Table~\ref{table:data}. 
Although it is possible to stream some image data at higher resolution or framerate, because there is a user interface running on the HoloLens and the HoloLens has limited computational resources, stream extra data will consume more energy and may result in headset overheating. 
The actual streamed frame rate may be lower due to the packet drop during streaming.
Hand tracking and eye tracking data are also streamed from the user interface app running on the HoloLens.
The eye tracking data consists of a 3D position which is the gaze origin and a 3D direction which is the gaze direction. 
The hand tracking data consists of 26 joint points for each hand. 
Each joint point contains a 3D position, and a quaternion indicates the orientation.
The point cloud is reconstructed using the RGB frames and depth frames.

\michael{mention how the point cloud data looks like and that it is registered (cite something, if possible)}

\begin{table}[]
\caption{Description of streamed data from HoloLens~2 image sensors.}
\centering
\begin{tabular}{lllr}
\toprule
Sensor                     & Resolution       & Format      & Framerate \\
\midrule
RGB camera                 & 760 $\times$ 428 & RGB8        & 7.5\,fps           \\
Depth camera               & 640 $\times$ 480 & Grayscale8  & 1\,fps             \\
Infrared active brightness & 320 $\times$ 288 & Grayscale8  & 5\,fps             \\
Infrared depth             & 320 $\times$ 288 & Depth16     & 5\,fps \\
\bottomrule
\end{tabular}
\label{table:data}
\end{table}



% D1 - 
% D2 - 
% D3 - 
% E1 - 
% E2 - 
